A Puff of Steem: Security Analysis of Decentralized Content Curation

Decentralized content curation is the process through which uploaded posts are ranked and filtered based exclusively on users' feedback. Platforms such as the blockchain-based Steemit employ this type of curation while providing monetary incentives to promote the visibility of high quality posts according to the perception of the participants. Despite the wide adoption of the platform very little is known regarding its performance and resilience characteristics. In this work, we provide a formal model for decentralized content curation that identifies salient complexity and game-theoretic measures of performance and resilience to selfish participants. Armed with our model, we provide a first analysis of Steemit identifying the conditions under which the system can be expected to correctly converge to curation while we demonstrate its susceptibility to selfish participant behaviour. We validate our theoretical results with system simulations in various scenarios.

==> acknowledgements.tex <==
\section{Acknowledgements}
  We thank Edith Elkind, Professor at the University of Oxford, for her guidance on relevant previous academic work.
  We also acknowledge the help and recommendations from Kousha Etessami, Professor at the University of Edinburgh, in order to prove the convergence bound of Steem.

  We would also like to extend our gratitude to Steemit's blogger @jga, Juli\'an Gonz\'alez. His blog posts~\cite{curationRewards,selfvoters} analyzing Steem internals have been of invaluable help for our understanding of the system.


==> algs.tex <==
\section{Steem post voting system procedures}
  \label{appendix:procs}
  \subimport{./algorithms/}{steeminitalg.tex}
  \subimport{./algorithms/}{steemauxalg.tex}
  \subimport{./algorithms/}{steemhandlevotealg.tex}
  \subimport{./algorithms/}{steemvotealg.tex}


==> conclusion.tex <==
\section{Conclusion}
  Keep inventing new decentralized content curation platforms.


==> steemhonestinitalg.tex <==
\begin{algorithm}[H]
  \caption{$\textsc{Init}^{\honest}\left(\stpowvec, \attspan, \pid,
  \rounds, a, b, c\right)$}
  \label{alg:steem:init:honest}
  \begin{algorithmic}[1]
    \State Store input parameters as constants
    \State $\mathrm{votedPosts} \gets \emptyset$
  \end{algorithmic}
\end{algorithm}

